Gradient Obfuscation Gives a False Sense of Security in Federated Learning

Federated learning has been proposed as a privacy-preserving machine learning framework that enables multiple clients to collaborate without sharing raw data. However, client privacy protection is not guaranteed by design in this framework. Prior work has shown that the gradient sharing strategies in federated learning can be vulnerable to data reconstruction attacks. In practice, though, clients may not transmit raw gradients considering the high communication cost or due to privacy enhancement requirements. Empirical studies have demonstrated that gradient obfuscation, including intentional obfuscation via gradient noise injection and unintentional obfuscation via gradient compression, can provide more privacy protection against reconstruction attacks. In this work, we present a new data reconstruction attack framework targeting the image classification task in federated learning. We show that commonly adopted gradient postprocessing procedures, such as gradient quantization, gradient sparsification, and gradient perturbation, may give a false sense of security in federated learning. Contrary to prior studies, we argue that privacy enhancement should not be treated as a byproduct of gradient compression. Additionally, we design a new method under the proposed framework to reconstruct the image at the semantic level. We quantify the semantic privacy leakage and compare with conventional based on image similarity scores. Our comparisons challenge the image data leakage evaluation schemes in the literature. The results emphasize the importance of revisiting and redesigning the privacy protection mechanisms for client data in existing federated learning algorithms.

==> sections/experiments.tex <==
\section{Experiments with Various Settings}\label{section:experiments}

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/experiments/latent_dim.pdf}
    \caption{
    Gradient distance versus the optimization iteration when changing the dimension $d_z$ of the vectorization of the latent representation $\Z_{m,i}$.
    The three schemes based on latent weight projection converge faster than the baseline ``No Projection'', which can be treated as using an identity function with $d_{z} = 49,\!152$.  
    When $d_z$ further decreases, the convergence becomes slower.  
    }
    \label{fig:effect_dim}
\end{figure}

\begin{figure}[!tb]
    \begin{overpic}[width=\linewidth, height=1.9\linewidth]{figs/5x4.pdf}
        \put(10, 90){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/16/4_ori.png}}
        \put(20.5, 90){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/16/4_recon.png}}
        \put(31.5, 90){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/16/5_ori.png}}
        \put(42, 90){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/16/5_recon.png}}
    
        \put(10, 79.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/16/11_ori.png}}
        \put(20.5, 79.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/16/11_recon.png}}
        \put(31.5, 79.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/16/15_ori.png}}
        \put(42, 79.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/16/15_recon.png}}
        %===========================================================
        \put(10, 78){\includegraphics[width=0.8\linewidth, height=1.3pt]{figs/lines/line.png}}
        \put(10, 67){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/32/0_ori.png}}
        \put(20.5, 67){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/32/0_recon.png}}
        \put(31.5, 67){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/32/9_ori.png}}
        \put(42, 67){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/32/9_recon.png}}

        \put(10, 56.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/32/18_ori.png}}
        \put(20.5, 56.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/32/18_recon.png}}
        \put(31.5, 56.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/32/24_ori.png}}
        \put(42, 56.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/32/24_recon.png}}
        %===========================================================
        \put(10, 55){\includegraphics[width=0.8\linewidth, height=1.3pt]{figs/lines/line.png}}
        \put(10, 44){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/64/21_ori.png}}
        \put(20.5, 44){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/64/21_recon.png}}
        \put(31.5, 44){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/64/32_ori.png}}
        \put(42, 44){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/64/32_recon.png}}

        \put(10, 33.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/64/56_ori.png}}
        \put(20.5, 33.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/64/56_recon.png}}
        \put(31.5, 33.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/64/58_ori.png}}
        \put(42, 33.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/64/58_recon.png}}
        %===========================================================
        \put(10, 32){\includegraphics[width=0.8\linewidth, height=1.3pt]{figs/lines/line.png}}
        \put(10, 21){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/128/99_ori.png}}
        \put(20.5, 21){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/128/99_recon.png}}
        \put(31.5, 21){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/128/85_ori.png}}
        \put(42, 21){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/128/85_recon.png}}

        \put(10, 10.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/128/115_ori.png}}
        \put(20.5, 10.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/128/115_recon.png}}
        \put(31.5, 10.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/128/118_ori.png}}
        \put(42, 10.5){\includegraphics[width=0.19\linewidth]{figs/experiments/batch/128/118_recon.png}}

        \put(0,90){\intab[0.68]{Batch Size $16$}}
        \put(0,88){\intab[0.68]{LPIPS: $0.188$}}
        \put(0,67){\intab[0.68]{Batch Size $32$}}
        \put(0,65){\intab[0.68]{LPIPS: $0.236$}}
        \put(0,44){\intab[0.68]{Batch Size $64$}}
        \put(0,42){\intab[0.68]{LPIPS: $0.270$}}
        \put(0,21){\intab[0.68]{Batch Size $128$}}
        \put(0,19){\intab[0.68]{LPIPS: $0.297$}}   
    \end{overpic}
    \vspace*{-50pt}
    \caption{
    Pairs of the original image and the reconstructed results for different local batch settings. 
    Increasing the batch size will reduce the reconstruction quality. 
    A large batch size does not provide a complete privacy protection. 
    \label{fig:impact_batch_size}
    }
\end{figure}

In this section, we investigate the proposed ROG attack with various settings and parameters in FedAvg.
We first explore the effect of the dimension of the latent representation $\Z_{m,i}$, and then provide discussions on the reconstruction results when the federated learning models and hyperparameters are changed. 
The experimental settings are the same as those in Section~\ref{section:realization} unless otherwise noted.

\highlight{Dimension of Latent Representation }
In this experiment, we train three autoencoders~\cite{baldi2012autoencoders} to obtain different encoding functions $\enc(\cdot)$ and the decoding functions $\dec(\cdot)$ in the ROG attack. 
For the three autoencoders, we set the dimension $d_z$ of the vectorization of the latent representation $\Z_{m,i}$ to $8192$, $2048$, and $512$, respectively. 
In the reconstruction attack, the dimension $d_z$ is equal to the number of unknown variables that an adversary wants to inspect. 
A smaller $d_z$ can improve the solvability of the system for the attacker, but may lead to more information loss during the encoding and decoding procedure. 
For the baseline method without projection, the number of unknown variables is equal to the number of pixels in the images. 
In our study, where each RGB image has a resolution of $128\times 128$, the number of unknowns is $49,\!152$.  
The optimization curves of different attack schemes are shown in Figure~\ref{fig:effect_dim}. 
It can be observed that the three methods with the autoencoder projection converge faster than the baseline method without projection.  
When the dimension $d_z$ decreases, the convergence rate is reduced. 
The results confirm the effectiveness of the latent vector projection in ROG.  
As it is difficult to find good encoding and decoding functions with little information loss, the dimension $d_{z}$ should not be set too small. 
On the other hand, a large $d_z$ will increase the memory consumption and reduce the solvability of the system. 

\begin{figure}[!tb]
    \begin{overpic}[width=\linewidth]{figs/4x4.pdf}
    \put(17, 69){\includegraphics[width=0.2\linewidth]{figs/experiments/round/10/0_ori.png}}
    \put(38, 69){\includegraphics[width=0.2\linewidth]{figs/experiments/round/10/1_ori.png}}
    \put(59, 69){\includegraphics[width=0.2\linewidth]{figs/experiments/round/10/5_ori.png}}
    \put(80, 69){\includegraphics[width=0.2\linewidth]{figs/experiments/round/10/14_ori.png}}

    \put(17, 67){\includegraphics[width=0.83\linewidth, height=1.3pt]{figs/lines/line.png}}

    \put(17, 45){\includegraphics[width=0.2\linewidth]{figs/experiments/round/10/0_recon.png}}
    \put(38, 45){\includegraphics[width=0.2\linewidth]{figs/experiments/round/10/1_recon.png}}
    \put(59, 45){\includegraphics[width=0.2\linewidth]{figs/experiments/round/10/5_recon.png}}
    \put(80, 45){\includegraphics[width=0.2\linewidth]{figs/experiments/round/10/14_recon.png}}

    \put(17, 24){\includegraphics[width=0.2\linewidth]{figs/experiments/round/30/0_recon.png}}
    \put(38, 24){\includegraphics[width=0.2\linewidth]{figs/experiments/round/30/1_recon.png}}
    \put(59, 24){\includegraphics[width=0.2\linewidth]{figs/experiments/round/30/5_recon.png}}
    \put(80, 24){\includegraphics[width=0.2\linewidth]{figs/experiments/round/30/14_recon.png}}

    \put(17, 3){\includegraphics[width=0.2\linewidth]{figs/experiments/round/50/0_recon.png}}
    \put(38, 3){\includegraphics[width=0.2\linewidth]{figs/experiments/round/50/1_recon.png}}
    \put(59, 3){\includegraphics[width=0.2\linewidth]{figs/experiments/round/50/5_recon.png}}
    \put(80, 3){\includegraphics[width=0.2\linewidth]{figs/experiments/round/50/14_recon.png}}

    \put(0, 76){\zoom{Raw Image}}
    \put(0, 55){\zoom{$K=10$}}
    \put(0, 51){\zoom{LPIPS $0.277$}}
    \put(0, 35.5){\zoom{$K=30$}}
    \put(0, 31.5){\zoom{LPIPS $0.338$}}
    \put(0, 16){\zoom{$K=50$}}
    \put(0, 12){\zoom{LPIPS $0.645$}}
    \end{overpic}
    \vspace*{-20pt}
    \caption{
    Reconstructed images at different communication round $K$. 
    As the number of communication rounds increases, the model weight gets closer to the local minimum and the magnitude of the gradient shrinks. 
    As a result, the attack becomes more difficult.   
    \label{fig:attack_round}}
\end{figure}



\highlight{Client Batch Size}
We choose the client batch size from $\{16, 32, 64, 128\}$ and present the reconstruction results in Figure~\ref{fig:impact_batch_size}. 
Intuitively, averaging the gradients over a larger batch gives more privacy protection. 
However, we can observe that a larger batch size does not completely prevent privacy leakage. 
When the batch size is increased, the averaging effect on the gradient will have an impact on the reconstructed results. 
For example, when the batch size is $128$, the reconstructed image of the Jeep has a different foreground but shares the background with the original image.   
A similar pattern can be observed in the image pairs of the cinema building and the snoek fish.  
On the other hand, the average LPIPS value is relatively low, which implies that the overall reconstructions resemble the raw images. 
We conclude that although increasing the batch size reduces the reconstruction quality, it may not be viewed as a good privacy enhancement strategy.  
A comprehensive study of large batch training with batch normalization is left for future work. 

\highlight{Different Communication Rounds }
In previous discussions, we exploit the vulnerabilities of using a randomly initialized neural network model in FedAvg.  
As the number of communication rounds increases, the neural network model weight gets closer to the local minimum and the gradient norm will decrease. 
The attack scheme may obtain trivial solutions when the magnitude of the shared gradient diminishes with the communication round. 
We empirically examine the reconstruction results by using the model with communication round $K \in \{10, 30, 50\}$.  
The attack results are shown in Figure~\ref{fig:attack_round}.
It can be observed that as the number $K$ of communication round increases, the reconstruction quality is reduced and the attack results gradually become unrecognizable. 
The observations suggest that it is more effective for the attacker to reconstruct data at the early stage of federated learning. 

\begin{figure}[!tb]
    \begin{overpic}[width=\linewidth]{figs/4x4.pdf}
    \put(17, 69){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/lenet/0_ori.png}}
    \put(38, 69){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/lenet/5_ori.png}}
    \put(59, 69){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/lenet/6_ori.png}}
    \put(80, 69){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/lenet/13_ori.png}}

    \put(17, 67){\includegraphics[width=0.83\linewidth, height=1.3pt]{figs/lines/line.png}}

    \put(17, 45){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/lenet/0_recon.png}}
    \put(38, 45){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/lenet/5_recon.png}}
    \put(59, 45){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/lenet/6_recon.png}}
    \put(80, 45){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/lenet/13_recon.png}}

    \put(17, 24){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/vgg/0_recon.png}}
    \put(38, 24){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/vgg/5_recon.png}}
    \put(59, 24){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/vgg/6_recon.png}}
    \put(80, 24){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/vgg/13_recon.png}}

    \put(17, 3){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/resnet/0_recon.png}}
    \put(38, 3){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/resnet/5_recon.png}}
    \put(59, 3){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/resnet/6_recon.png}}
    \put(80, 3){\includegraphics[width=0.2\linewidth]{figs/experiments/arch/resnet/13_recon.png}}

    \put(0, 76){\zoom{Raw Image}}
    \put(0, 55){\zoom{LeNet}}
    \put(0, 51){\zoom{LPIPS $0.173$}}
    \put(0, 35.5){\zoom{VGG-7}}
    \put(0, 31.5){\zoom{LPIPS $0.193$}}
    \put(0, 16){\zoom{ResNet-18}}
    \put(0, 12){\zoom{LPIPS $0.291$}}
    \end{overpic}
    \vspace*{-20pt}
    \caption{
    Attack against different neural network architectures. 
    All reconstructed images are visually similar to raw images. 
    \label{fig:attack_arch}}
\end{figure}

\highlight{Neural Network Architectures }
In this experiment, we study the impact of different neural network architectures on the attack scheme. 
We choose the LeNet, VGG-7, and ResNet-18 and demonstrate the reconstruction results in Figure~\ref{fig:attack_arch}. 
LeNet is a five-layer convolutional network with $5\times5$ kernels, and VGG-7 is a seven-layer convolutional network with $3\times3$ kernels.
ResNet-18 is an eighteen-layer residual network with skip connections. 
Intuitively, the increased number of nodes in a neural network appears to give the adversary more advantages, as the number of known conditions will also increase.  
On the other hand, more sophisticated neural network architecture will have an increased nonlinearity, thus impeding a successful reconstruction.  
In Figure~\ref{fig:attack_arch}, we can observe that all reconstructed images under different neural network architectures are visually similar. 
Our observation is consistent with the prior study that changing the neural network architecture may not directly affect the privacy protection level. 
A more extensive study concerning neural network architectures is warranted in future work. 


